Winding Through: Crowd Navigation via Topological Invariance

We focus on robot navigation in crowded environments. The challenge of predicting the motion of a crowd around a robot makes it hard to ensure human safety and comfort. Recent approaches often employ end-to-end techniques for robot control or deep architectures for high-fidelity human motion prediction. While these methods achieve important performance benchmarks in simulated domains, dataset limitations and high sample complexity tend to prevent them from transferring to real-world environments. Our key insight is that a low-dimensional representation that captures critical features of crowd-robot dynamics could be sufficient to enable a robot to wind through a crowd smoothly. To this end, we mathematically formalize the act of passing between two agents as a rotation, using a notion of topological invariance. Based on this formalism, we design a cost functional that favors robot trajectories contributing higher passing progress and penalizes switching between different sides of a human. We incorporate this functional into a model predictive controller that employs a simple constant-velocity model of human motion prediction. This results in robot motion that accomplishes statistically significantly higher clearances from the crowd compared to state-of-the-art baselines while maintaining competitive levels of efficiency, across extensive simulations and challenging real-world experiments on a self-balancing robot.

==> archived/ballbot-model.tex <==
\subsection{Ballbot Model}

\cmnote{possibly compress this section further}

%A ballbot consists of a mechanical body that dynamically balances over an omnidirectional spherical wheel (ball) that makes single-point contact with the ground (see \figref{fig:ballbot-model}).

Fix a global frame $G = \{\hat{x}, \hat{y}, \hat{z}\}$. A ballbot consists of a mechanical body with mass $M$ and moment of inertia $I_0$ that dynamically balances over an omnidirectional spherical wheel (ball) of mass $m$ and radius $r$ that makes single-point contact with the ground (see \figref{fig:ballbot-model}). Denote by
\begin{equation}
    c_1 = \begin{pmatrix}
    x_1 & y_1 & z_1
    \end{pmatrix}^{\intercal}
    = c_2 + h\begin{pmatrix}
    \sin\theta_1^x &
    \sin\theta_1^y &
    \cos\theta_1^x
    \end{pmatrix}^{\intercal}\mbox{,}
\end{equation}
the position of the body's center of mass (CoM), where $\left(\theta_1^x, \theta_1^y\right)$ represent the inclination of the body from $\hat{z}$ about the $\hat{y}$ and $\hat{x}$ axes respectively and
\begin{equation}
    c_2 = \begin{pmatrix}
    x_2 & y_2 & z_2
    \end{pmatrix}^{\intercal}
    = r \begin{pmatrix}
    \theta_1^x + \theta_2^x & 
    \theta_1^y + \theta_2^y &
    1
    \end{pmatrix}^{\intercal}
\end{equation}
describes the position of the ball's CoM. 

Denote by $q = \begin{pmatrix}\theta_1^x & \dot{\theta}_1^x & \dot{x}_1 & \theta_1^y & \dot{\theta}_1^y & \dot{y}_1\end{pmatrix}^\intercal$ the state of the robot body. Considering a sampling time of size $T$, we may derive the discretized linearized equations of motion for the ballbot body about the equilibrium $(\theta_1^x, \dot{\theta}_1^x, \theta_1^y, \dot{\theta}_1^y)\approx 0$ as:
\begin{equation}
        q_{k+1} = A_{d}q_k+B_{d}u_k,\qquad
        p_k =  C_{d}q_k\mbox{,}
\end{equation}
where $A_d = \exp(AT)$, $B_d = (\exp(AT)-I)B$ and 
\begin{equation}
A = 
    \begin{pmatrix}
        A_{0} & 0\\0 & A_0
    \end{pmatrix}\mbox{,}\quad    B = \begin{pmatrix}
        B_0 & 0\\0 & B_0
    \end{pmatrix}
\end{equation}
where
\begin{equation}
    A_0 =
    \begin{pmatrix}
        0 & 1 & 0\\
        a & 0 & 0\\
        a(r+h) & 0 & 0
    \end{pmatrix}\mbox{,}
    \quad
    B_0 = \begin{pmatrix}
        0\\ -b\\ r - (r+h)b
    \end{pmatrix}\mbox{,}
\end{equation}
and
\begin{equation}
    \begin{split}
        a = & \frac{Mgh}{2 + M(r+ h)^2 + mr^2}\mbox{,}\\
        b = & \frac{Mr(r + h) + mr^2}{I_0 + M(r+ h)^2 + mr^2}
    \end{split}\mbox{.}
\end{equation}
Finally, $C_d = I$, i.e., the state is fully observable, $u = \begin{pmatrix}\ddot{\theta}_2^x & \ddot{\theta}_2^y\end{pmatrix}^\intercal$ is the control input and $k \in\mathbb{N}$ is a timestep count.



For body stabilization and velocity control, we adopt a State Feedback Control (SFC) architecture of the form $u_k = K\left(q_k - \tilde{q}\right)$ where $K$ is a gain matrix acquired with the LQR technique and $\tilde{q}$ represents a reference\footnote{Note that around the equilibrium, it holds that $\theta^x_1, \theta^y_1\approx 0$ and therefore $v^x = \dot{x}_1\approx \dot{x}_2$ and $v^y = \dot{y}_1\approx \dot{y}_2$.} of the form $\tilde{q} = \begin{pmatrix}0 & 0 & v^x & 0 & 0 & v^y\end{pmatrix}^\intercal$ where $v^x = \dot{x}_1$, $v^y = \dot{y}_1$. This results in closed-loop dynamics of the form 
\begin{equation}
    q_{k+1} = g_c(q_k,\tilde{q}) = (A_d-B_{d}K)q_{k} + B_{d}K\tilde{q}\mbox{.}\label{eq:sfc}
\end{equation}

In this work, we employ the velocity control architecture of \citet{yamane2019} who place an integral controller on top of SFC to account for steady-state errors through due to e.g., floor conditions, robot design parameters etc. For more details on the control design, please refer to the patent of \citet{yamane2019}.

==> archived/ballbot.tex <==
\section{Application}\label{sec:implementation}

To illustrate the value of T-MPC, we apply it on a ballbot. In this section, we introduce a ballbot model and augment T-MPC to account for the ballbot's stabilization and velocity-control constraints.

%\kbnote{Introduction to the high-level implementation details we will cover in this section. Describe the "full state" and "observable state".}

%\kbnote{Should we use rollout or trajectory? Are there instances where we should use rollout over trajectory?}



% Fix a global frame $G = \{\hat{x}, \hat{y}, \hat{z}\}$. A ballbot consists of a mechanical body with mass $M$ and moment of inertia $I_0$ that dynamically balances over an omnidirectional spherical wheel (ball) of mass $m$ and radius $r$ that makes single-point contact with the ground (see \figref{fig:ballbot-model}). 

% Denote by
% \begin{equation}
%     c_1 = \begin{pmatrix}
%     x_1 & y_1 & z_1
%     \end{pmatrix}^{\intercal}
%     = c_2 + h\begin{pmatrix}
%     \sin\theta_1^x &
%     \sin\theta_1^y &
%     \cos\theta_1^x
%     \end{pmatrix}^{\intercal}\mbox{,}
% \end{equation}
% the position of the body's center of mass (CoM), where $\left(\theta_1^x, \theta_1^y\right)$ represent the inclination of the body from $\hat{z}$ about the $\hat{y}$ and $\hat{x}$ axes respectively and
% \begin{equation}
%     c_2 = \begin{pmatrix}
%     x_2 & y_2 & z_2
%     \end{pmatrix}^{\intercal}
%     = r \begin{pmatrix}
%     \theta_1^x + \theta_2^x & 
%     \theta_1^y + \theta_2^y &
%     1
%     \end{pmatrix}^{\intercal}
% \end{equation}
% describes the position of the ball's CoM. 




%The closed-loop dynamics can be written in the form
% \begin{equation}
%     s_{k+1} = g(s_k,u_k) = (A_d-B_{d}K)s_{k} + B_{d}Ku_k\mbox{.}\label{eq:sfc}
% \end{equation}
% where $K$ is a gain matrix acquired with the LQR technique and $\tilde{s}_k$ represents a reference of the form $\tilde{s}_k = \tilde{s}(v_k) = \begin{pmatrix}v_k & 0 & 0 & 0 & 0\end{pmatrix}^\intercal$, expressing the specification that the ballbot needs to track a planar velocity $v$ while maintaining an upright pose.


%The ballbot's linearized dynamics about the vertical equilibrium can be written in the form $s_{k+1} = A_{d}s_k+B_{d}u_k$ where $A_d$ and $B_d$ are matrices of appropriate dimensions.

% where $A_d = \exp(AT)$, $B_d = (\exp(AT)-I)B$ and 
% \begin{equation}
% A = 
%     \begin{pmatrix}
%         A_{0} & 0\\0 & A_0
%     \end{pmatrix}\mbox{,}\quad    B = \begin{pmatrix}
%         B_0 & 0\\0 & B_0
%     \end{pmatrix}
% \end{equation}
% where
% \begin{equation}
%     A_0 =
%     \begin{pmatrix}
%         0 & 1 & 0\\
%         a & 0 & 0\\
%         a(r+h) & 0 & 0
%     \end{pmatrix}\mbox{,}
%     \quad
%     B_0 = \begin{pmatrix}
%         0\\ -b\\ r - (r+h)b
%     \end{pmatrix}\mbox{,}
% \end{equation}
% and
% \begin{equation}
%     \begin{split}
%         a = & \frac{Mgh}{2 + M(r+ h)^2 + mr^2}\mbox{,}\\
%         b = & \frac{Mr(r + h) + mr^2}{I_0 + M(r+ h)^2 + mr^2}
%     \end{split}\mbox{.}
% \end{equation}

%\footnote{Note that around the equilibrium, it holds that $\theta^x_1, \theta^y_1\approx 0$ and therefore $v^x = \dot{x}_1\approx \dot{x}_2$ and $v^y = \dot{y}_1\approx \dot{y}_2$.}



%$u_k = K\left(q_k - \tilde{q}\right)$ 

% \subsection{T-MPC on a Ballbot}

% We augment the T-MPC formulation incorporating the closed-loop dynamics of the ballbot. T-MPC searches for a \emph{reference} control trajectory $\tilde{\boldsymbol{v}}^*$ that upon executed on the ballbot's low-level controller will yield the desirable behavior:
% \begin{equation}
% \begin{split}
% \boldsymbol{v}^{*} = \arg & \min_{v_{0:N-1}} \mathcal{J}(s_{1:N}, s^{1}_{1:N}, \dots, s^{n}_{1:N})\\
%     s.t.\: & s_{k+1} = g(s_k, v_k)\\
%           & s^i_{k+1} = f(S_{k-h:k})\\
%   \label{eq:mpc}
% \end{split}\mbox{,}
% \end{equation}

% \begin{equation}
% \begin{split}
% \left(\boldsymbol{\tilde{v}}^{*}, \boldsymbol{s}^{*}\right) = \arg & \min_{\tilde{v}_{0:N-1}} \mathcal{J}(\boldsymbol{S})\\
%     s.t.\: & \tilde{v}_k \in \mathcal{V}\\
%           & S_0 = s_0 \cup_{i = 1:n} s_0^i\\
%           & v_k^i = \mathcal{O}(s_{k-h:k}^i)\\
%           & U_k = \tilde{v}_k \cup_{i=1:n} v_k^i\\
%           & S_{k+1} = F(S_{k}, U_k)\\
%           & \boldsymbol{S} = (S_1,\dots, S_N)\\
%           & \tilde{q}_k = \tilde{q}(\tilde{v}_k)\\
%           & q_{k+1} = g_c(q_k,\tilde{q}_k)\\
%   \label{eq:tmpcballbot}
% \end{split}\mbox{,}
% \end{equation}
% where we assume that the robot perfectly observes its own augmented state $q$.




% A sampling-based approach is used to generate robot trajectories that sample the set of all homotopy classes. Assuming the robot follows a policy, $\pi(s_k, v_k)$, we generate a set of $k$ trajectories, $\zeta_k$, for the robot by sampling goal destinations, $\tilde{g}_k$, a fixed distance, $d_k$, from the ego agent with heading $\theta_k$ and generate a  and augment\kbnote{(see fig TBD)}. In order to diversely sample the set of all homotopy classes, goal destinations are sampled with an angular uniform distribution from $\theta_k = 0$ to $\theta_k = 2\pi$. By integrating the topology reward into the MPC formulation, we reward trajectories that maximize the winding number across all pairwise agents, allowing the ego agent to optimize over safety, efficiency, and homotopy class.





%\cmnote{are we really sampling or are these subgoals fixed throughout control loops? Sampling often implies stochasticity.}\kbnote{we are not actually sampling subgoals, but by fixing these subgoals we effectively "sample" the set of all possible topologies. But there is nothing stochastic about the rollout generation.}






%To generate rollout $v^j$ at timestep $k$, we contrive a modified state, $\boldsymbol{\hat{s}}_k$, by sampling an ego agent goal destination, $\hat{s}_T$, a fixed distance, $d$, from the planar position of the ego agent with heading $\theta^j$. We assume the ego agent follows the policy $\pi(\boldsymbol{\hat{s}}_{k})$ and dynamic agents follow a linear policy, $\pi^i(s_k)$.

% $m$ rollouts $\boldsymbol{v}\in\mathcal{M}$.

%$\pi'_k (s'_0, v_k)$ at every timestep by sampling goal destinations, $\tilde{s}_t$, a fixed distance, $d_k$, from the ego agent with heading $\theta_k$ and generate a  and augment\kbnote{(see fig TBD)}.  

%By integrating the topology reward into the MPC formulation, we reward trajectories that maximize the winding number across all pairwise agents, allowing the ego agent to optimize over safety, efficiency, and homotopy class.




==> archived/dataplots.tex <==
\begin{figure*}
% Always try to place the figure on top of a column to save space
    \centering
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figs/ORCA-world-safety.png}
        \caption{Safety in ORCA world.}
        \label{fig:safety-orca}
    \end{subfigure}
    \\
    \begin{subfigure}{\linewidth}
     \centering
        \includegraphics[width=\linewidth]{figs/CADRL-world-safety.png}
        \caption{Safety in CADRL world.} 
         \label{fig:safety-cadrl}
     \end{subfigure}
\caption{Safety in different simulated worlds.\label{fig:safety-plots}}
\end{figure*}

\begin{figure*}
% Always try to place the figure on top of a column to save space
    \centering
    \begin{subfigure}{\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figs/ORCA-world-efficiency.png}
        \caption{Path time in ORCA world.}
    \end{subfigure}
    \\
    \begin{subfigure}{\linewidth}
     \centering
        \includegraphics[width=\linewidth]{figs/CADRL-world-efficiency.png}
        \caption{Path time in CADRL world.} 
         \label{fig:efficiency-cadrl}
     \end{subfigure}
\caption{Efficiency in different simulated worlds.\label{fig:efficiency-plots}}
\end{figure*}

==> archived/tables.tex <==
%------------------------------------------------------------------------------------- %
%---------------------------------- H1 ----------------------------------------------- %
%------------------------------------------------------------------------------------- %
\begin{table*}
\centering{%
{

\begin{tabular}{ccccccc}
\cline{1-7}
\multicolumn{1}{|c|}{\textbf{Number of Agents $\rightarrow$}} & \multicolumn{2}{c|}{Three} & \multicolumn{2}{c|}{Four} & \multicolumn{2}{c|}{Five} \\ \cline{1-7} 
\multicolumn{1}{|c|}{\textbf{Controller $\downarrow$}} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} \\ \cline{1-7} 
  
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{Linear VMPC} &
  \multicolumn{1}{c|}{\textbf{0.64}} &
  \multicolumn{1}{c|}{{10.87}} &
  \multicolumn{1}{c|}{\textbf{0.61}} &
  \multicolumn{1}{c|}{10.77} &
  \multicolumn{1}{c|}{\textbf{0.59}} &
  \multicolumn{1}{c|}{{11.27}} \\
\multicolumn{1}{|c|}{Linear TMPC} &
  \multicolumn{1}{c|}{\textbf{0.67}} &
  \multicolumn{1}{c|}{{\ul 10.6}} &
  \multicolumn{1}{c|}{\textbf{0.64}} &
  \multicolumn{1}{c|}{{\ul 10.44}} &
  \multicolumn{1}{c|}{\textbf{0.63}} &
  \multicolumn{1}{c|}{{\ul 10.94}} \\ \hline
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{CADRL VMPC} &
  \multicolumn{1}{c|}{\textbf{0.64}} &
  \multicolumn{1}{c|}{{12.61}} &
  \multicolumn{1}{c|}{\textbf{0.65}} &
  \multicolumn{1}{c|}{11.97} &
  \multicolumn{1}{c|}{\textbf{0.61}} &
  \multicolumn{1}{c|}{15.21} \\
\multicolumn{1}{|c|}{CADRL TMPC} &
  \multicolumn{1}{c|}{{\textbf{0.77}}} &
  \multicolumn{1}{c|}{11.15} &
  \multicolumn{1}{c|}{{\ul \textbf{0.75}}} &
  \multicolumn{1}{c|}{{11.09}} &
  \multicolumn{1}{c|}{\textbf{0.66}} &
  \multicolumn{1}{c|}{14.19} \\ \hline
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{ORCA VMPC} &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{{11.14}} &
  \multicolumn{1}{c|}{\textbf{0.66}} &
  \multicolumn{1}{c|}{11.66} &
  \multicolumn{1}{c|}{\textbf{0.65}} &
  \multicolumn{1}{c|}{{12.17}} \\
\multicolumn{1}{|c|}{ORCA TMPC} &
  \multicolumn{1}{c|}{{\ul 0.83}} &
  \multicolumn{1}{c|}{11.5} &
  \multicolumn{1}{c|}{\textbf{0.78}} &
  \multicolumn{1}{c|}{11.11} &
  \multicolumn{1}{c|}{{\ul \textbf{0.7}}} &
  \multicolumn{1}{c|}{12.66} \\ \hline
 
\end{tabular}

}
}
\caption{Topology Information in ORCA World}
\label{tab:H1}
\end{table*}

%------------------------------------------------------------------------------------- %
%---------------------------------- H1-C---------------------------------------------- %
%------------------------------------------------------------------------------------- %
\begin{table*}
\centering{%
{

\begin{tabular}{ccccccc}
\cline{1-7}
\multicolumn{1}{|c|}{\textbf{Number of Agents $\rightarrow$}} & \multicolumn{2}{c|}{Three} & \multicolumn{2}{c|}{Four} & \multicolumn{2}{c|}{Five} \\ \cline{1-7} 
\multicolumn{1}{|c|}{\textbf{Controller $\downarrow$}} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} \\ \cline{1-7} 
  
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{Linear VMPC} &
  \multicolumn{1}{c|}{\textbf{0.89}} &
  \multicolumn{1}{c|}{{\ul 11.56}} &
  \multicolumn{1}{c|}{\textbf{0.82}} &
  \multicolumn{1}{c|}{11.66} &
  \multicolumn{1}{c|}{\textbf{0.78}} &
  \multicolumn{1}{c|}{{\ul 10.15}} \\
\multicolumn{1}{|c|}{Linear TMPC} &
  \multicolumn{1}{c|}{\textbf{--}} &
  \multicolumn{1}{c|}{--} &
  \multicolumn{1}{c|}{\textbf{--}} &
  \multicolumn{1}{c|}{--} &
  \multicolumn{1}{c|}{\textbf{--}} &
  \multicolumn{1}{c|}{--} \\ \hline
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{CADRL VMPC} &
  \multicolumn{1}{c|}{\textbf{0.97}} &
  \multicolumn{1}{c|}{12.02} &
  \multicolumn{1}{c|}{\textbf{0.9}} &
  \multicolumn{1}{c|}{12.09} &
  \multicolumn{1}{c|}{\textbf{0.7}} &
  \multicolumn{1}{c|}{14.36} \\
\multicolumn{1}{|c|}{CADRL TMPC} &
  \multicolumn{1}{c|}{{\ul \textbf{1.17}}} &
  \multicolumn{1}{c|}{11.61} &
  \multicolumn{1}{c|}{{\ul \textbf{1.15}}} &
  \multicolumn{1}{c|}{{\ul 11.09}} &
  \multicolumn{1}{c|}{\textbf{0.85}} &
  \multicolumn{1}{c|}{12.64} \\ \hline
\multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{ORCA VMPC} &
  \multicolumn{1}{c|}{\textbf{0.98}} &
  \multicolumn{1}{c|}{{12.08}} &
  \multicolumn{1}{c|}{\textbf{0.92}} &
  \multicolumn{1}{c|}{12.32} &
  \multicolumn{1}{c|}{\textbf{0.79}} &
  \multicolumn{1}{c|}{13.38} \\
\multicolumn{1}{|c|}{ORCA TMPC} &
  \multicolumn{1}{c|}{\textbf{1.11}} &
  \multicolumn{1}{c|}{12.33} &
  \multicolumn{1}{c|}{\textbf{1.11}} &
  \multicolumn{1}{c|}{11.48} &
  \multicolumn{1}{c|}{{\ul \textbf{0.91}}} &
  \multicolumn{1}{c|}{12.88} \\ \hline
\end{tabular}

}
}
\caption{Topology Information in CADRL World}
\label{tab:H1-C}
\end{table*}


%------------------------------------------------------------------------------------- %
%---------------------------------- H2---------------------------------------------- %
%------------------------------------------------------------------------------------- %
\begin{table*}
\centering{%
{

\begin{tabular}{lcccccccccccc}
\cline{1-13}
\multicolumn{1}{|l|}{\textbf{Number of Agents $\rightarrow$}} &
  \multicolumn{4}{c|}{Three} &
  \multicolumn{4}{c|}{Four} &
  \multicolumn{4}{c|}{Five} \\ \cline{1-13} 
\multicolumn{1}{|l}{} &
  \multicolumn{2}{c|}{Safety} &
  \multicolumn{2}{c|}{Path Time} &
  \multicolumn{2}{c|}{Safety} &
  \multicolumn{2}{c|}{Path Time} &
  \multicolumn{2}{c|}{Safety} &
  \multicolumn{2}{c|}{Path Time} \\ \cline{1-13} 
\multicolumn{1}{|l|}{\textbf{Controller $\downarrow$}} &
  ORCA &
  \multicolumn{1}{c|}{CADRL} &
  ORCA &
  \multicolumn{1}{c|}{CADRL} &
  ORCA &
  \multicolumn{1}{c|}{CADRL} &
  ORCA &
  \multicolumn{1}{c|}{CADRL} &
  ORCA &
  CADRL &
  ORCA &
  \multicolumn{1}{c|}{CADRL} \\ \cline{1-13} 
 &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{{\ul }} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{{\ul }} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \hline
\multicolumn{1}{|c|}{Linear VMPC} &
  \textbf{0.64} &
  \multicolumn{1}{c|}{0.89} &
  \textbf{10.87} &
  \multicolumn{1}{c|}{11.56} &
  \textbf{0.61} &
  \multicolumn{1}{c|}{0.82} &
  10.77 &
  \multicolumn{1}{c|}{11.66} &
  \textbf{0.59} &
  \multicolumn{1}{c|}{0.78} &
  11.27 &
  \multicolumn{1}{c|}{10.15} \\
\multicolumn{1}{|c|}{Linear TMPC} &
  \textbf{0.67} &
  \multicolumn{1}{l|}{} &
  10.6 &
  \multicolumn{1}{l|}{} &
  \textbf{0.64} &
  \multicolumn{1}{l|}{} &
  10.44 &
  \multicolumn{1}{l|}{} &
  \textbf{0.63} &
  \multicolumn{1}{l|}{} &
  10.94 &
  \multicolumn{1}{l|}{} \\ \hline
 &
  \multicolumn{4}{l}{\textbf{}} &
  \multicolumn{4}{l}{\textbf{}} &
  \multicolumn{4}{l}{} \\ \hline
\multicolumn{1}{|c|}{CADRL} &
  {0.68} &
  \multicolumn{1}{c|}{0.98} &
  \multicolumn{1}{l}{\; 9.82} &
  \multicolumn{1}{c|}{{10.75}} &
  \multicolumn{1}{l}{\; 0.63} &
  \multicolumn{1}{c|}{0.93} &
  10.34 &
  \multicolumn{1}{c|}{{\ul 10.26}} &
  0.6 &
  \multicolumn{1}{c|}{0.74} &
  12.32 &
  \multicolumn{1}{c|}{12.53} \\
\multicolumn{1}{|l|}{\quad \; CADRL VMPC} &
  0.64 &
  \multicolumn{1}{c|}{0.97} &
  12.61 &
  \multicolumn{1}{c|}{12.02} &
  0.64 &
  \multicolumn{1}{c|}{0.9} &
  11.97 &
  \multicolumn{1}{c|}{12.09} &
  0.61 &
  \multicolumn{1}{c|}{0.7} &
  15.21 &
  \multicolumn{1}{c|}{14.36} \\
\multicolumn{1}{|c|}{CADRL TMPC} &
  \textbf{0.77} &
  \multicolumn{1}{c|}{{\ul 1.17}} &
  \textbf{11.15} &
  \multicolumn{1}{c|}{11.61} &
  \textbf{0.77} &
  \multicolumn{1}{c|}{{\ul 1.15}} &
  11.09 &
  \multicolumn{1}{c|}{11.09} &
  0.66 &
  \multicolumn{1}{c|}{0.85} &
  14.19 &
  \multicolumn{1}{c|}{12.64} \\ \hline
 &
  \multicolumn{4}{l}{\textbf{}} &
  \multicolumn{4}{l}{{\ul \textbf{}}} &
  \multicolumn{4}{l}{} \\ \hline
\multicolumn{1}{|c|}{ORCA} &
  \textbf{0.67} &
  \multicolumn{1}{c|}{0.91} &
  {\ul 9.33} &
  \multicolumn{1}{c|}{{\ul 10.65}} &
  0.64 &
  \multicolumn{1}{c|}{0.78} &
  {\ul 9.7} &
  \multicolumn{1}{c|}{11.03} &
  \textbf{0.61} &
  \multicolumn{1}{c|}{0.69} &
  {\ul 10.08} &
  \multicolumn{1}{c|}{{\ul 11.63}} \\
\multicolumn{1}{|l|}{\quad \: \, ORCA VMPC} &
  0.74 &
  \multicolumn{1}{c|}{0.98} &
  11.14 &
  \multicolumn{1}{c|}{12.08} &
  0.66 &
  \multicolumn{1}{c|}{0.92} &
  11.66 &
  \multicolumn{1}{c|}{12.32} &
  \textbf{0.65} &
  \multicolumn{1}{c|}{0.79} &
  12.17 &
  \multicolumn{1}{c|}{13.38} \\
\multicolumn{1}{|c|}{ORCA TMPC} &
  {\ul 0.83} &
  \multicolumn{1}{c|}{1.11} &
  11.5 &
  \multicolumn{1}{c|}{12.33} &
  {\ul \textbf{0.78}} &
  \multicolumn{1}{c|}{1.11} &
  11.11 &
  \multicolumn{1}{c|}{11.48} &
  {\ul \textbf{0.7}} &
  \multicolumn{1}{c|}{{\ul 0.91}} &
  12.66 &
  \multicolumn{1}{c|}{12.88} \\ \hline
\end{tabular}
}
}
\caption{CADRL and ORCA Worlds}
\label{tab:H2}
\end{table*}

%------------------------------------------------------------------------------------- %
%---------------------------------- H3---------------------------------------------- %
%------------------------------------------------------------------------------------- %
\begin{table*}
\centering{%

\begin{tabular}{ccccccc}
\cline{1-7}
\multicolumn{1}{|c|}{\textbf{Number of Agents $\rightarrow$}} & \multicolumn{2}{c|}{Three} & \multicolumn{2}{c|}{Four} & \multicolumn{2}{c|}{Five} \\ \cline{1-7} 
\multicolumn{1}{|c|}{\textbf{Controller $\downarrow$}} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} \\ \cline{1-7} 
                               &              &             &             &             &             &             \\ \hline
\multicolumn{1}{|c|}{CADRL} &
  \multicolumn{1}{c|}{{0.98}} &
  \multicolumn{1}{c|}{{\ul 10.75}} &
  \multicolumn{1}{c|}{{0.93}} &
  \multicolumn{1}{c|}{\ul 10.26} &
  \multicolumn{1}{c|}{{0.74}} &
  \multicolumn{1}{c|}{{\ul 12.53}} \\
\multicolumn{1}{|c|}{ORCA} &
  \multicolumn{1}{c|}{{0.91}} &
  \multicolumn{1}{c|}{10.65} &
  \multicolumn{1}{c|}{{0.78}} &
  \multicolumn{1}{c|}{11.03} &
  \multicolumn{1}{c|}{{0.69}} &
  \multicolumn{1}{c|}{11.63} \\
\multicolumn{1}{|c|}{CADRL TMPC} &
  \multicolumn{1}{c|}{{\ul 1.17}} &
  \multicolumn{1}{c|}{11.61} &
  \multicolumn{1}{c|}{{\ul 1.15}} &
  \multicolumn{1}{c|}{11.09} &
  \multicolumn{1}{c|}{{0.85}} &
  \multicolumn{1}{c|}{12.64} \\
\multicolumn{1}{|c|}{ORCA TMPC} &
  \multicolumn{1}{c|}{{1.11}} &
  \multicolumn{1}{c|}{12.33} &
  \multicolumn{1}{c|}{{1.11}} &
  \multicolumn{1}{c|}{11.48} &
  \multicolumn{1}{c|}{{\ul 0.91}} &
  \multicolumn{1}{c|}{12.88} \\ \hline
\end{tabular}
}
\caption{CADRL and ORCA vs TMPC in CADRL World}
\label{tab:H3-C}
\end{table*}


%------------------------------------------------------------------------------------- %
%---------------------------------- H3-C---------------------------------------------- %
%------------------------------------------------------------------------------------- %
\begin{table*}
\centering{%
{

\begin{tabular}{ccccccc}
\cline{1-7}
\multicolumn{1}{|c|}{\textbf{Number of Agents $\rightarrow$}} & \multicolumn{2}{c|}{Three} & \multicolumn{2}{c|}{Four} & \multicolumn{2}{c|}{Five} \\ \cline{1-7} 
\multicolumn{1}{|c|}{\textbf{Controller $\downarrow$}} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} &
  \multicolumn{1}{c|}{Safety} &
  \multicolumn{1}{c|}{Path Time} \\ \cline{1-7} 
 &
   &
   &
   &
   &
   &
   \\ \hline
\multicolumn{1}{|c|}{CADRL} &
  \multicolumn{1}{c|}{{0.68}} &
  \multicolumn{1}{c|}{{\ul 9.82}} &
  \multicolumn{1}{c|}{{0.63}} &
  \multicolumn{1}{c|}{10.34} &
  \multicolumn{1}{c|}{{0.6}} &
  \multicolumn{1}{c|}{{\ul 12.32}} \\
\multicolumn{1}{|c|}{ORCA} &
  \multicolumn{1}{c|}{{0.67}} &
  \multicolumn{1}{c|}{9.33} &
  \multicolumn{1}{c|}{{0.64}} &
  \multicolumn{1}{c|}{{\ul 9.7}} &
  \multicolumn{1}{c|}{{0.61}} &
  \multicolumn{1}{c|}{10.08} \\
\multicolumn{1}{|c|}{CADRL TMPC} &
  \multicolumn{1}{c|}{{0.77}} &
  \multicolumn{1}{c|}{11.15} &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{11.09} &
  \multicolumn{1}{c|}{{0.66}} &
  \multicolumn{1}{c|}{14.19} \\
\multicolumn{1}{|c|}{ORCA TMPC} &
  \multicolumn{1}{c|}{{\ul {0.83}}} &
  \multicolumn{1}{c|}{11.5} &
  \multicolumn{1}{c|}{{\ul {0.78}}} &
  \multicolumn{1}{c|}{11.11} &
  \multicolumn{1}{c|}{{\ul {0.7}}} &
  \multicolumn{1}{c|}{12.66} \\ \hline
\end{tabular}

}
}
\caption{CADRL and ORCA vs TMPC in ORCA World}
\label{tab:H3}
\end{table*}


\begin{table*}
\centering
\resizebox{\columnwidth}{!}{%
\addvbuffer[0pt 2pt]{
\begin{tabular}{lccccccc}
%\cline{1-19}
\toprule
\multicolumn{1}{l}{Scenario} & \multicolumn{3}{c}{One Agent} & \multicolumn{2}{c}{Two Agents} & \multicolumn{1}{c}{Three Agents} \\ 
\midrule
Interaction & & Sequential1 & Concurrent1 & Sequential2 & Concurrent2 & Sequential3 & Concurrent3\\

%\multicolumn{1}{l|}{CARLA Autopilot} & \xmark & \multicolumn{1}{C}{\checkmark} &  &  &  &  \\ \hline
% \multicolumn{1}{l}{Metric} & \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &h
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$}\\

\midrule
\multicolumn{1}{l|}{\multirow{4}{*}{CADRL}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} & 
\multicolumn{1}{c|}{$81.57 \pm 8.85$} &
\multicolumn{1}{c|}{$72.34 \pm 12.91$} &
\multicolumn{1}{c|}{$84.83 \pm 8.31$} &
\multicolumn{1}{c|}{$90.07 \pm 10.84$} &
\multicolumn{1}{c|}{$85.52 \pm 5.82$} &
\multicolumn{1}{c}{$86.69 \pm 2.63$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} & 
\multicolumn{1}{c|}{$14.47 \pm 0.96$} &
\multicolumn{1}{c|}{$15.59 \pm 1.96$} &
\multicolumn{1}{c|}{$14.52 \pm 2.32$} &
\multicolumn{1}{c|}{$12.69 \pm 1.90$} &
\multicolumn{1}{c|}{$14.96 \pm 1.18$} &
\multicolumn{1}{c}{$12.26 \pm 0.89$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} & 
\multicolumn{1}{c|}{$3.04 \pm 0.22$} &
\multicolumn{1}{c|}{$2.20 \pm 0.28$} &
\multicolumn{1}{c|}{$3.14 \pm 0.08$} &
\multicolumn{1}{c|}{$3.05 \pm 0.12$} &
\multicolumn{1}{c|}{$3.18 \pm 0.13$} &
\multicolumn{1}{c}{$2.78 \pm 0.06$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2)$} & 
\multicolumn{1}{c|}{$1.09 \pm 0.73$} &
\multicolumn{1}{c|}{$1.11 \pm 0.54$} &
\multicolumn{1}{c|}{$1.81 \pm 1.49$} &
\multicolumn{1}{c|}{$1.42 \pm 0.51$} &
\multicolumn{1}{c|}{$1.32 \pm 0.66$} &
\multicolumn{1}{c}{$1.40 \pm 0.51$}\\
\midrule

\multicolumn{1}{l|}{\multirow{4}{*}{MPC}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} & 
\multicolumn{1}{c|}{$96.58 \pm 1.05$} &
\multicolumn{1}{c|}{$90.64 \pm 0.81$} &
\multicolumn{1}{c|}{$82.43 \pm 6.92$} &
\multicolumn{1}{c|}{$90.40 \pm 1.28$} &
\multicolumn{1}{c|}{$84.04 \pm 0.52$} &
\multicolumn{1}{c}{$80.82 \pm 3.09$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} & 
\multicolumn{1}{c|}{$12.35 \pm 0.77$} &
\multicolumn{1}{c|}{$11.35 \pm 0.78$} &
\multicolumn{1}{c|}{$14.76 \pm 1.33$} &
\multicolumn{1}{c|}{$11.42 \pm 0.61$} &
\multicolumn{1}{c|}{$14.74 \pm 0.85$} &
\multicolumn{1}{c}{$13.63 \pm 0.68$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} &
\multicolumn{1}{c|}{$2.93 \pm 0.19$} &
\multicolumn{1}{c|}{$2.47 \pm 0.08$} &
\multicolumn{1}{c|}{$3.33 \pm 0.11$} &
\multicolumn{1}{c|}{$3.19 \pm 0.07$} &
\multicolumn{1}{c|}{$3.26 \pm 0.12$} &
\multicolumn{1}{c}{$3.08 \pm 0.04$}\\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2)$} & 
\multicolumn{1}{c|}{$1.63 \pm 0.54$} &
\multicolumn{1}{c|}{$1.22 \pm 0.44$} &
\multicolumn{1}{c|}{$1.75 \pm 0.65$} &
\multicolumn{1}{c|}{$1.36 \pm 0.43$} &
\multicolumn{1}{c|}{$1.68 \pm 0.48$} &
\multicolumn{1}{c}{$1.70 \pm 0.48$}\\
\midrule


\multicolumn{1}{l|}{\multirow{4}{*}{\textbf{CADRL+MPC}}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} &
\multicolumn{1}{c|}{$\mathbf{85.07 \pm 3.22}$}&
\multicolumn{1}{c|}{$\mathbf{88.54 \pm 1.79}$} &
\multicolumn{1}{c|}{$\mathbf{82.47 \pm 2.07}$} &
\multicolumn{1}{c|}{$\mathbf{90.61 \pm 1.43}$} &
\multicolumn{1}{c|}{$\mathbf{79.78 \pm 2.22}$} &
\multicolumn{1}{c}{$\mathbf{78.40 \pm 2.05}$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} &
\multicolumn{1}{c|}{$\mathbf{12.77 \pm 0.74}$}&
\multicolumn{1}{c|}{$\mathbf{12.01 \pm 1.37}$} &
\multicolumn{1}{c|}{$\mathbf{13.33 \pm 0.27}$} &
\multicolumn{1}{c|}{$\mathbf{11.16 \pm 0.75}$} &
\multicolumn{1}{c|}{$\mathbf{15.13 \pm 0.92}$} &
\multicolumn{1}{c}{$\mathbf{14.06 \pm 2.32}$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} & 
\multicolumn{1}{c|}{$\mathbf{3.26 \pm 0.14}$} &
\multicolumn{1}{c|}{$\mathbf{2.50 \pm 0.16}$} &
\multicolumn{1}{c|}{$\mathbf{3.35 \pm 0.11}$} &
\multicolumn{1}{c|}{$\mathbf{3.21 \pm 0.08}$} &
\multicolumn{1}{c|}{$\mathbf{3.44 \pm 0.08}$} &
\multicolumn{1}{c}{$\mathbf{3.08 \pm 0.18}$} \\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2) $} & 
\multicolumn{1}{c|}{$\mathbf{1.32 \pm 0.75}$} &
\multicolumn{1}{c|}{$\mathbf{1.22 \pm 0.63}$} &
\multicolumn{1}{c|}{$\mathbf{1.47 \pm 0.52}$} &
\multicolumn{1}{c|}{$\mathbf{1.37 \pm 0.72}$} &
\multicolumn{1}{c|}{$\mathbf{2.04 \pm 1.27}$} &
\multicolumn{1}{c}{$\mathbf{2.22 \pm 1.16}$} \\


\bottomrule
%\multicolumn{1}{l|}{MPC + MFP} & \multicolumn{1}{l}{} &  &  &  &  &  \\ \hline
\end{tabular}
}
}
\caption{Simulated evaluation}
\label{tab:sim-results}
\end{table*}

\begin{table*}
\centering
\resizebox{\columnwidth}{!}{%
\addvbuffer[0pt 2pt]{
\begin{tabular}{lccccccc}
%\cline{1-19}
\toprule
\multicolumn{1}{l}{Scenario} & \multicolumn{3}{c}{One Agent} & \multicolumn{2}{c}{Two Agents} & \multicolumn{1}{c}{Three Agents} \\ 
\midrule
Interaction & & Sequential1 & Concurrent1 & Sequential2 & Concurrent2 & Sequential3 & Concurrent3\\

%\multicolumn{1}{l|}{CARLA Autopilot} & \xmark & \multicolumn{1}{C}{\checkmark} &  &  &  &  \\ \hline
% \multicolumn{1}{l}{Metric} & \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &h
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$} &
% \multicolumn{1}{c}{$\mathcal{T}$ (s)} &
% \multicolumn{1}{c}{$\mathcal{C}$}\\

\midrule
\multicolumn{1}{l|}{\multirow{4}{*}{CADRL}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} & 
\multicolumn{1}{c|}{$81.57 \pm 8.85$} &
\multicolumn{1}{c|}{$72.34 \pm 12.91$} &
\multicolumn{1}{c|}{$84.83 \pm 8.31$} &
\multicolumn{1}{c|}{$90.07 \pm 10.84$} &
\multicolumn{1}{c|}{$85.52 \pm 5.82$} &
\multicolumn{1}{c}{$86.69 \pm 2.63$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} & 
\multicolumn{1}{c|}{$14.47 \pm 0.96$} &
\multicolumn{1}{c|}{$15.59 \pm 1.96$} &
\multicolumn{1}{c|}{$14.52 \pm 2.32$} &
\multicolumn{1}{c|}{$12.69 \pm 1.90$} &
\multicolumn{1}{c|}{$14.96 \pm 1.18$} &
\multicolumn{1}{c}{$12.26 \pm 0.89$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} & 
\multicolumn{1}{c|}{$3.04 \pm 0.22$} &
\multicolumn{1}{c|}{$2.20 \pm 0.28$} &
\multicolumn{1}{c|}{$3.14 \pm 0.08$} &
\multicolumn{1}{c|}{$3.05 \pm 0.12$} &
\multicolumn{1}{c|}{$3.18 \pm 0.13$} &
\multicolumn{1}{c}{$2.78 \pm 0.06$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2)$} & 
\multicolumn{1}{c|}{$1.09 \pm 0.73$} &
\multicolumn{1}{c|}{$1.11 \pm 0.54$} &
\multicolumn{1}{c|}{$1.81 \pm 1.49$} &
\multicolumn{1}{c|}{$1.42 \pm 0.51$} &
\multicolumn{1}{c|}{$1.32 \pm 0.66$} &
\multicolumn{1}{c}{$1.40 \pm 0.51$}\\
\midrule

\multicolumn{1}{l|}{\multirow{4}{*}{MPC}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} & 
\multicolumn{1}{c|}{$96.58 \pm 1.05$} &
\multicolumn{1}{c|}{$90.64 \pm 0.81$} &
\multicolumn{1}{c|}{$82.43 \pm 6.92$} &
\multicolumn{1}{c|}{$90.40 \pm 1.28$} &
\multicolumn{1}{c|}{$84.04 \pm 0.52$} &
\multicolumn{1}{c}{$80.82 \pm 3.09$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} & 
\multicolumn{1}{c|}{$12.35 \pm 0.77$} &
\multicolumn{1}{c|}{$11.35 \pm 0.78$} &
\multicolumn{1}{c|}{$14.76 \pm 1.33$} &
\multicolumn{1}{c|}{$11.42 \pm 0.61$} &
\multicolumn{1}{c|}{$14.74 \pm 0.85$} &
\multicolumn{1}{c}{$13.63 \pm 0.68$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} &
\multicolumn{1}{c|}{$2.93 \pm 0.19$} &
\multicolumn{1}{c|}{$2.47 \pm 0.08$} &
\multicolumn{1}{c|}{$3.33 \pm 0.11$} &
\multicolumn{1}{c|}{$3.19 \pm 0.07$} &
\multicolumn{1}{c|}{$3.26 \pm 0.12$} &
\multicolumn{1}{c}{$3.08 \pm 0.04$}\\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2)$} & 
\multicolumn{1}{c|}{$1.63 \pm 0.54$} &
\multicolumn{1}{c|}{$1.22 \pm 0.44$} &
\multicolumn{1}{c|}{$1.75 \pm 0.65$} &
\multicolumn{1}{c|}{$1.36 \pm 0.43$} &
\multicolumn{1}{c|}{$1.68 \pm 0.48$} &
\multicolumn{1}{c}{$1.70 \pm 0.48$}\\
\midrule


\multicolumn{1}{l|}{\multirow{4}{*}{\textbf{CADRL+MPC}}} & 
\multicolumn{1}{c|}{$\mathcal{L} (\%)$} &
\multicolumn{1}{c|}{$\mathbf{85.07 \pm 3.22}$}&
\multicolumn{1}{c|}{$\mathbf{88.54 \pm 1.79}$} &
\multicolumn{1}{c|}{$\mathbf{82.47 \pm 2.07}$} &
\multicolumn{1}{c|}{$\mathbf{90.61 \pm 1.43}$} &
\multicolumn{1}{c|}{$\mathbf{79.78 \pm 2.22}$} &
\multicolumn{1}{c}{$\mathbf{78.40 \pm 2.05}$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{T} (s)$} &
\multicolumn{1}{c|}{$\mathbf{12.77 \pm 0.74}$}&
\multicolumn{1}{c|}{$\mathbf{12.01 \pm 1.37}$} &
\multicolumn{1}{c|}{$\mathbf{13.33 \pm 0.27}$} &
\multicolumn{1}{c|}{$\mathbf{11.16 \pm 0.75}$} &
\multicolumn{1}{c|}{$\mathbf{15.13 \pm 0.92}$} &
\multicolumn{1}{c}{$\mathbf{14.06 \pm 2.32}$}\\

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{D} (m)$} & 
\multicolumn{1}{c|}{$\mathbf{3.26 \pm 0.14}$} &
\multicolumn{1}{c|}{$\mathbf{2.50 \pm 0.16}$} &
\multicolumn{1}{c|}{$\mathbf{3.35 \pm 0.11}$} &
\multicolumn{1}{c|}{$\mathbf{3.21 \pm 0.08}$} &
\multicolumn{1}{c|}{$\mathbf{3.44 \pm 0.08}$} &
\multicolumn{1}{c}{$\mathbf{3.08 \pm 0.18}$} \\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$\mathcal{A} (m/s^2) $} & 
\multicolumn{1}{c|}{$\mathbf{1.32 \pm 0.75}$} &
\multicolumn{1}{c|}{$\mathbf{1.22 \pm 0.63}$} &
\multicolumn{1}{c|}{$\mathbf{1.47 \pm 0.52}$} &
\multicolumn{1}{c|}{$\mathbf{1.37 \pm 0.72}$} &
\multicolumn{1}{c|}{$\mathbf{2.04 \pm 1.27}$} &
\multicolumn{1}{c}{$\mathbf{2.22 \pm 1.16}$} \\


\bottomrule
%\multicolumn{1}{l|}{MPC + MFP} & \multicolumn{1}{l}{} &  &  &  &  &  \\ \hline
\end{tabular}
}
}
\caption{Experimental evaluation}
\label{tab:results}
\end{table*}

==> sections/acknowledgment.tex <==
\section*{Acknowledgments}
This work was (partially) funded by the National Science Foundation IIS (\#2007011), National Science Foundation DMS (\#1839371), the Office of Naval Research, US Army Research Laboratory CCDC, Amazon, and Honda Research Institute USA.
